An unstructured finite-volume level set / front tracking method for two-phase flows with large density-ratios

We extend the unstructured LEvel set / froNT tracking (LENT) method for handling two-phase flows with strongly different densities (high-density ratios) by providing the theoretical basis for the numerical consistency between the mass and momentum conservation in the collocated Finite Volume discretization of the single-field two-phase Navier-Stokes equations. Our analysis provides the theoretical basis for the mass conservation equation introduced by Ghods and Herrmann [3] and used in [4, 5, 6, 7, 8]. We use a mass flux that is consistent with mass conservation in the implicit Finite Volume discretization of the two-phase momentum convection term, and solve the single-field Navier-Stokes equations with our SAAMPLE segregated solution algorithm [2]. The proposed $\rho$LENT method recovers exact numerical stability for the two-phase momentum advection of a spherical droplet with density ratios ranging in $[1, 10^4]$. Numerical stability is demonstrated for in terms of the relative $L_\infty$ velocity error norm, for density-ratios in the range of $[1, 10^4]$, dynamic viscosity-ratios in the range of $[1, 10^4]$ and very strong surface tension forces, for challenging mercury/air and water/air fluid pairings. In addition, the solver performs well in cases characterized by strong interaction between two phases, i.e., oscillating droplets and rising bubbles. The proposed $\rho$LENT method is applicable to any other two-phase flow simulation method that discretizes the single-field two-phase Navier-Stokes Equations using the collocated unstructured Finite Volume Method but does not solve an advection equation for the phase indicator using a flux-based approach, by adding the proposed geometrical approximation of the mass flux and the auxiliary mass conservation equation to the solution algorithm.

==> credit-statement.tex <==
\section*{CRediT author statement}

\begin{description}

\item Jun Liu: Conceptualization, Methodology, Software, Validation, Investigation, Writing - Original Draft, Writing - Review \& Editing, Visualization 

\item Tobias Tolle: Conceptualization, Methodology, Software, Formal analysis, Investigation, Validation, Data Curation, Writing - Original Draft, Writing - Review \& Editing 

\item Dieter Bothe: Writing - Review \& Editing, Formal analysis, Funding acquisition

\item Tomislav Mari\'c: Conceptualization, Methodology, Software, Formal analysis, Investigation, Validation, Data Curation, Writing - Original Draft, Writing - Review \& Editing, Supervision, Funding acquisition

\end{description}


==> research-highlights.tex <==
\section*{Highlights}

\begin{itemize}
    \item Exact numerical consistency recovered for the two-phase momentum convection. 
    \item Theoretical basis provided for the use of the auxiliary mass conservation equation.
    \item Provided a strict relationship between the mass flux density and the phase indicator.
    \item Implicit discretization of the two-phase momentum convective term.
    \item Increased numerical stability with large surface tension forces and density-ratios.
\end{itemize}


==> sections/laplace-beltrami.tex <==
\section{Implicit discretization of the Laplace-Beltrami operator using unstructured FVM}
\label{sec:lapl}

\subsection{Laplace-Beltrami operator for implicit surfaces}

The derivation of the Laplace-Beltrami operator for implicit surfaces given by \citet[Appendix A]{Bertalmio2001} is based on variational calculus applied to the minimization problem of the following functional 

\todo[inline]{Jun: APPENDIX A in \citet{Bertalmio2001} hier abtyppen, ich werde die Zwischenschritte noch beschreiben die in der Herleitung fehlen}

\subsection{Discretization using the unstructured finite volume method}

\begin{equation}
    \partial_t u = 
        \frac{1}{\|\nabla\phi\|}\nabla\cdot
        \left(
            \Projection(\nabla{u})\|\nabla\phi\|
        \right)
    \label{eq:laplacebeltramivol}
\end{equation}

is the Laplace-Beltrami equation expressed using volume operators, where $P_{\nabla\phi}\nabla{u}$ is the projection operator
%
\begin{equation}
    \Projection(\nabla u) :=  \nabla{u} -
    \frac{\nabla{u}\cdot\nabla\phi}{\|\nabla\phi\|^2}\nabla\phi\|\nabla\phi\|
    \label{eq:pnablaphi}
\end{equation}
%
that projects $\nabla u$ tangentially onto $\Interface$.

The discretization of \cref{eq:laplacebeltramivol} using the unstructured Finite Volume Method (FVM) starts with the integration over the cell $\Cell{c}$
%
\begin{equation}
    \int_{\Cell{c}} \partial_t u \|\nabla\phi\| \, dV = 
    \int_{\Cell{c}} \nabla\cdot
        \left(
            P_{\nabla\phi}\nabla{u}\left\|\nabla\phi\right\|
        \right) \, dV \, dt.
    \label{eq:lb-int}
\end{equation}
%
The l.h.s. term of \cref{eq:lb-int} is discretized as
%
\begin{equation}
    \int_{\Cell{c}} \partial_t u \|\nabla\phi\| \, dV \approx  
    (\partial_t u)_c \|\nabla\phi\|_c |\Cell{c}|, 
\end{equation}
%
with second-order accuracy\todo{Cite Hirsch}, and the divergence term on the r.h.s. of \cref{eq:lb-int} is reformulated as  
%
\begin{equation}
    \begin{aligned}
        \int_{\Cell{c}} \nabla\cdot (\Projection(\nabla u) \|\nabla\phi\|)\, dV  & =  
        \int_{\Cell{c}} \nabla\cdot\left(\left[\nabla u- \frac{\nabla u\cdot\nabla\phi}{\|\nabla\phi\|^2}\nabla\phi\right]\|\nabla\phi\|\right) \, dV\\
        & = \int_{\Cell{c}} \nabla\cdot\left(\|\nabla\phi\|\nabla u\right)\, dV - 
            \int_{\Omega{c}}\ \nabla\cdot\left(\frac{\nabla u\cdot\nabla\phi}{\|\nabla\phi\|}\nabla\phi\right), dV. 
    \end{aligned}
    \label{eq:divproj}
\end{equation}
%
It is clear that the first term on the r.h.s.\ in the last line of \cref{eq:divproj} is a standard Laplacian (diffusion) term, that can be discretized using the unstructured FVM. However, the coefficient $\|\nabla \phi\|$ makes this diffusion operator anisotropic, unless $\phi$ is a signed distance field, in which case $\|\nabla \phi\|=1$. Note that $\|\nabla \phi\|$ can possibly abruptly change in the near vicinity of $\Interface$, and this must be carefully considered on the discrete level. The second term on the r.h.s.\ in the last line of \cref{eq:divproj} requires further reformulation. 

The boundary of a cell $\partial\Cell{c}$, 
%
\begin{equation}
    \partial\Cell{c} :=\bigcup_{f \in F_c} S_f,
\end{equation}
%
is defined as a union of continuous surfaces, so-called \emph{faces} $S_f$. This leads to  
%
\begin{align}
      \int_{\Cell{c}} \nabla\cdot\left(\frac{\nabla u \cdot\nabla\phi}{\|\nabla\phi\|}\nabla\phi\right)dV 
        & = \int_{\partial\Cell{c}}\frac{\nabla u \cdot\nabla\phi}{\|\nabla\phi\|}\nabla\phi\cdot\Vec{n}ds \nonumber \\
        & = \sum_{f\in F_{C}}\frac{(\nabla u )_{f}\cdot(\nabla\phi)_{f}}{\|\nabla\phi\|_f}(\nabla\phi)_{f}\cdot\Sf \nonumber \\
        & = \sum_{f\in F_{C}}\frac{(\nabla\phi)_{f}\cdot(\nabla u )_{f}}{\|\nabla\phi\|_f}(\nabla\phi)_{f}\cdot\Sf,
\end{align}
%
as the unstructured FVM averages values at centroids of $S_f$ with second-order accuracy\todo{cite Hirsch}. 

\begin{figure}[!htb]
    \centering
    \def\svgwidth{0.5\textwidth}
    \input{figures/LBO.pdf_tex}\notag\\
    \caption{Decomposition of $\nabla\phi$ into orthogonal and non-orthogonal contribution.}
    \label{fig:phigrad-decomp}
\end{figure}

\begin{equation}
    \nabla\phi_{f}=\nabla\phi_{f,\perp}+\nabla\phi_{f,\parallel}\\
\end{equation}

\begin{equation}
    (\nabla u )_{f}^{n+1}\cdot(\nabla\phi)_{f}^{n} =
        (\nabla u )_{f}^{n+1}\cdot(\nabla\phi)_{f,\perp}^{n} + (\nabla u )_{f}^{n+1}\cdot(\nabla\phi)_{f,\parallel}^{n}
\end{equation}

\begin{equation}
    \begin{aligned}
        (\nabla u )_{f}^{n+1}\cdot(\nabla\phi)_{f,\perp}^{n} 
        & = (\nabla u )_{f}^{n+1} \cdot [ (\nabla\phi^n\cdot\Sfhat) \Sfhat] \\
      & = (\nabla u )_{f}^{n+1}\cdot\Sfhat\frac{\left\|\df\right\|}{\left\|\df\right\|}.(\nabla\phi)^n_{f}\cdot\Sfhat\\
      & = (\nabla u )_{f}^{n+1}\cdot\df\cdot\frac{(\nabla\phi)^n_{f}\cdot\Sfhat}{\left\|\df\right\|}\\
      & = \left( u _{N_{f}}^{n+1}- u _{C_{f}}^{n+1}\right)\cdot\frac{(\nabla\phi)^n_{f}\cdot\Sfhat}{\left\|\df\right\|}\\
    \end{aligned}
\end{equation}

\begin{equation}
    (\nabla u )_{f}^{m}\cdot(\nabla\phi)_{f,\parallel}^{n} = \left(\omega_{f}\nabla u _{N_{f}}^{m} + (1-\omega_{f})\nabla u _{C_{f}}^{m}\right)\cdot\left((\nabla\phi)_{f} - (\nabla\phi)_{f,\perp}\right), \quad m = 1,2,3,\dots
\end{equation}

\begin{equation}
    \begin{aligned}
    \sum_{f\in F_{C}}\frac{(\nabla u )_{f}\cdot(\nabla\phi)_{f}}{\|\nabla\phi\|}(\nabla\phi)_{f}\cdot\Sf
    & =\underbrace{\sum_{f\in F_{C}}
    \left(u_{N_{f}}^{n+1}-u_{O_{f}}^{n+1}\right)\cdot\frac{(\nabla\phi)_{f}\cdot\Sfhat}{\left\|\df\right\|}\cdot\frac{(\nabla\phi)_{f}\cdot\Sf}{\|\nabla\phi\|_{f}}}_{\text{IMPLICIT PART}}\\
    & +\underbrace{\sum_{f\in F_{C}}\left(\omega_{f}\nabla u _{N_{f}}^{m} + (1-\omega_{f})\nabla u _{O_{f}}^{m}\right)\cdot\left((\nabla\phi)_{f} - (\nabla\phi)_{f,\perp}\right)\cdot\frac{\nabla\phi_{f}\cdot\Sf}{\left\|\nabla\phi\right\|_{f}}}_{\text{EXPLICIT PART}}
    \end{aligned}
\end{equation}





==> sections/results-laplace-beltrami.tex <==
\section{Results}
\label{sec:res}

$Test\ case\ 1$. In the first case a simple condition is considered , namely computing a stationary sphere. As an analytical comparsion the Laplace-Beltrami equation $-\Delta_{\Sigma}c^{\Sigma} + c^{\Sigma} = f(\boldsymbol{x})$ on $\Sigma$ is chosen, which has a unique analytical solution for given $f(\boldsymbol{x})$. With the specific $f(\boldsymbol{x})$\\
%
\begin{equation}
    f(\boldsymbol{x}) = a(3x_{1}^{2}x_{2}-x_{2}^{3})
\end{equation}\\
%
when $a=-\frac{13}{8}\sqrt{\frac{35}{\pi}}$, then $c^{\Sigma}$ can be solved (see \cite{aubin1982nonlinear}) as \\
%
\begin{equation}
    c^{\Sigma}(\boldsymbol{x})= a\frac{|\boldsymbol{x}|^2}{12+|\boldsymbol{x}|^2}(3x_{1}^{2}x_{2}-x_{2}^{3})
\end{equation}\\
%
The sphere has radius $r = 1\,m$. Trigonal and polygonal surface meshes are used to resolve the sphere's surface. In the computation $c^{\Sigma}$ indicates the concentration distribution of a surface quantity on the sphere surface $\Sigma$. To compare the numerical results and analytical solution two error norms $L^1$ and $L^2$ are adopted, whose definitions are denoted as\\
%
\begin{equation}
    L^1 = \frac{\sum_{f}\left | \phi_{analytical}^{\Sigma}-\phi_{num}^{\Sigma}\right |\boldsymbol{A}_{f}}{\sum_{f}\boldsymbol{A}_{f}}
\end{equation}
%
%
\begin{equation}
    L^2 = \sqrt{\frac{\sum_{f}\left | \phi_{analytical}^{\Sigma}-\phi_{num}^{\Sigma}\right |^2\boldsymbol{A}_{f}}{\sum_{f}\boldsymbol{A}_{f}}}
\end{equation}\\
%
respectively. \\
$[results\ description]$\\
$Test\ case\ 2$. The surface mesh in this case undergoes translation and deformation. A sphere of radius $r=0.25\,m$ translates in a cuboid of size $l=5\,m$, $w=2\,m$ and $h=2\,m$ with velocity $\boldsymbol{u}(t)$, which is given by\\
%
\begin{equation}
\label{eq:velocity_sphere}
    \boldsymbol{u}(t)=\boldsymbol{u}^{\infty}\sin{\omega t}
\end{equation}\\
%
with ${u}^{\infty}=(0.1,0,0)ms^{-1}$,$\omega=0.0051/s$. For $c^{\Sigma}$, it is predefined by\\
%
\begin{equation}
\label{eq:concentration_profile}
    c^{\Sigma}(\boldsymbol{x})=c^{\Sigma}_{0}|x_{1}|
\end{equation}\\
%
, constant $c^{\Sigma}_{0}$ is given by $1\,mol\,m^{-2}$. A new error norm called relative mass error is applied, which is interpreted by\\
%
\begin{equation}
    \epsilon_{rel}=\frac{\sum_{f}\left |\left (c_{i}^{\Sigma}\right )_{P}S_{P} - \left (c_{analytical}^{\Sigma}\right )_{P} S_{P} \right |}{\left (\rho_{analytical}^{\Sigma}\right )_{P} S_{P}}
\end{equation}\\
%
$[results\ description]$\\
$Test\ case\ 3$.
A more complex condition based on case 2 is developed in this test case. Which is, a diffusive transport of $c^{\Sigma}$ takes place on surface of the sphere of radius $r=0.25m$. The transport equation is defined as\\
%
\begin{equation}
    \partial_{t}c_{i}^{\Sigma}-D\Delta_{\Sigma}c_{i}^{\Sigma}=0
\end{equation}
%
The sphere translates as presented in Eq.\ref{eq:velocity_sphere} and the concentration profile $c^{\Sigma}$ is predefined as stated by Eq.\ref{eq:concentration_profile}. The diffusion coefficient is given as $D=0.001\,m^{2}\,s^{-1}$.\\
$[results\ description]$\\
$Test\ case\ 4$.
This test case is based on test case 1. The advancement is that the translation defined by Eq.\ref{eq:velocity_sphere} is added to the sphere of radius $r=1\,m$. The center position of the sphere, for the sake of simplification, is initially set to origin.\\ 
$[results\ description]$\\
$Test\ case\ 5$.
For evaluation of the transport on surface under substantial deformation, a test case as described in \cite{leveque1996high} is implemented.A sphere of radius $r=0.15\,m$ moves in a cube of $1\,m$.The movement of the sphere starts with the center position $(0.35,0.35,0.35)$. The concentration profile $c^{\Omega}$ is initialized as a constant $1\,mol\,m^{-2}$. The sphere deforms with the velocity field $\boldsymbol{u}=(u_{x},u_{y},u_{z})$, which is defined as\\
%
\begin{equation}
    \begin{split}
       u_{x}& = 2\sin^{2}(\pi x)\sin{2\pi y}\sin{2\pi z}\cos{\pi t}\\
       u_{y}& = -\sin(2\pi x)\sin^{2}{\pi y}\sin{2\pi z}\cos{\pi t}\\
       u_{z}& = -\sin(2\pi x)\sin{2\pi y}\sin^{2}{\pi z}\cos{\pi t}
    \end{split}
\end{equation}
%
$[results\ description]$\\









==> significance-and-novelties.tex <==
\section*{Significance and Novelty}

Two-phase flows involving incompressible phases with very different densities (high-density ratios) still pose a significant challenge to contemporary numerical two-phase flow simulation methods. Consequently, there has been an increase in scientific publications taking on this challenge. Most publications focus on structured domain discretization and the staggered variable arrangement. For the first time, a numerically consistent discretization for the momentum convection term in the two-phase single-field Navier-Stokes equations is achieved using the implicit collocated Finite Volume discretization together with the hybrid Level Set / Front Tracking method. Another novel aspect of the manuscript is the theoretical basis for the auxiliary mass conservation equation, used throughout the literature. We also show a strict relationship between the mass-flux density and the phase indicator, which does not leave much freedom in evaluating the mass-flux density when ensuring consistency with a single-cell-layer phase indicator (e.g., the volume fraction). The proposed method also applies to other collocated Finite Volume two-phase flow methods, with the slight difference in the computation of the mass-flux density from the approximation of the fluid interface. 



